PST900: RGB-Thermal Calibration, Dataset and Segmentation Network

In this work we propose long wave infrared (LWIR) imagery as a viable supporting modality for semantic segmentation using learning-based techniques. We first address the problem of RGB-thermal camera calibration by proposing a passive calibration target and procedure that is both portable and easy to use. Second, we present PST900, a dataset of 894 synchronized and calibrated RGB and Thermal image pairs with per pixel human annotations across four distinct classes from the DARPA Subterranean Challenge. Lastly, we propose a CNN architecture for fast semantic segmentation that combines both RGB and Thermal imagery in a way that leverages RGB imagery independently. We compare our method against the state-of-the-art and show that our method outperforms them in our dataset.

==> pages/extras.tex <==
\subsection{Multimodal Stereo}

Treible \etal proposed a novel stereo dataset comprising of thermal-thermal, color-color and thermal-color stereo pairs with LiDAR ground truth data \cite{treible2017cats}. They highlight the need for tools and algorithms to work on thermal specific data and stress the challenges involved in using traditional color image based algorithms on the low-texture, low-resolution and comparatively nosier thermal imagery, here in the context of stereo depth estimation. The dataset was collected of static scenes with a 3D LiDAR for ground truth in a variety of environmental conditions such as night-time, day-time and fog. In their experiments with cross modal depth estimation, they highlight the difficulty in distilling information from one modality to the other, primarily in the context of stereo disparity estimation but also with regards to cross modal matching in general.

Recently, \cite{beaupre2019siamese} proposed a patch-wise disparity estimation CNN for thermal-rgb cross modal disparity estimation with the focus on person detection and depth estimation. They evaluate their method on LITIV \cite{torabi2012iterative} and St. Charles data-sets \cite{bilodeau2014thermal}. They further the highlight the difficulties associated with cross modal matching and also showed that in some cases a descriptor based method for cross modal matching outperformed their CNN architecture.

In the domain of person detection, Kristoffersen \etal proposed a classical key-point detection and clustering based method of pedestrian detection \cite{kristoffersen2016pedestrian} using DBSCAN clustering and then a Kalman Filter to track pedestrian groups. A stereo pair of LWIR cameras is used to identify clusters in 3D and track them. Depth is known only at the sparse key-point locations.

Prakash \etal propose an alternative view to stereo matching in thermal image space by matching isotherms instead of raw thermal intensity values \cite{prakash20063d}. Isotherms are lines connecting points of equal temperature. A push broom approach is used to sweep through all temperature values present in the image  data and identify intersections of isotherms and epipolar lines..
